Data-Driven Template-Free Invariant Generation

Automatic verification of concurrent programs faces state explosion due to the exponential possible interleavings of its sequential components coupled with large or infinite state spaces. An alternative is deductive verification, where given a candidate invariant, we establish inductive invariance and show that any state satisfying the invariant is also safe. However, learning (inductive) program invariants is difficult. To this end, we propose a data-driven procedure to synthesize program invariants, where it is assumed that the program invariant is an expression that characterizes a (hopefully tight) over-approximation of the reachable program states. The main ideas of our approach are: (1) We treat a candidate invariant as a classifier separating states observed in (sampled) program traces from those speculated to be unreachable. (2) We develop an enumerative, template-free approach to learn such classifiers from positive and negative examples. At its core, our enumerative approach employs decision trees to generate expressions that do not over-fit to the observed states (and thus generalize). (3) We employ a runtime framework to monitor program executions that may refute the candidate invariant; every refutation triggers a revision of the candidate invariant. Our runtime framework can be viewed as an instance of statistical model checking, which gives us probabilistic guarantees on the candidate invariant. We also show that such in some cases, our counterexample-guided inductive synthesis approach converges (in probability) to an overapproximation of the reachable set of states. Our experimental results show that our framework excels in learning useful invariants using only a fraction of the set of reachable states for a wide variety of concurrent programs.

==> sections/conclusion.tex <==
InvGen is an automated and practical framework for observing
non-deterministic system behaviors and generating accurate system
properties. The approach is data-driven, leveraging counter-examples
and speculative negative states to guide the refinement process. The
learning model is template-free and decision-tree-based. One key
advantage of our framework is its independence from any known system
specifications or properties.

Future work includes multiple promising directions. First, exploring
alternative speculative sampling techniques enhances the convergence
of the learning process. Second, the decision tree learning method
could be further investigated, including the separator selection and
the exploit-exploration trade-off.


==> sections/related-old.tex <==
\noindent\textbf{Related Work on Invariant Generation} There are many different approaches to learn program invariants that
have been proposed in the literature.  Invariant synthesis using theorem provers is a formal method for automatically deriving invariants by symbolic executions and using mathematical reasoning and logical deduction to verify the correctness of the program. Vampire\cite{vampire} is a theorem prover and is designed for multiple advanced applications, such as satisfiability checking and program analysis. The method for automatic generation of a specific type of invariants \cite{tp_v} is based on the automatic analysis of the update predicates of loops and the theorem prover Vampire. Besides, a theorem prover\cite{almostcorrect} are normally used for validity check for invariance properties of systems. Theorem proving tools are able to reason formally about data and relationships. However, these techniques are normally not able to give much useful feedback by generating counterexamples.

% For instance, the work on \jyo{implication cause learning}
% (ICE~\cite{garg2014ice} and ICE-DT~\cite{icedt}) is inspired by
% computational learning theory; the authors use a learner and a
% teacher, where the learner iteratively refines a candidate invariant
% using counterexamples provided by the teacher until a valid invariant
% is discovered.  \jyo{This line is still not clear. Where do these
% implications come from?} A central step is to include implications in
% the learning algorithm that guarantee that the learned invariant is
% inductive. Checking if a candidate invariant is inductive requires the
% use of a model checker or an SMT solver.  In \cite{padon2016ivy}, the
% authors employ counterexamples provided by the Ivy model checker to
% learn inductive invariants using DistAI: an enumerative method over
% data traces. DistAI also requires the user to supply safety properties
% and a model checker to vet candidate invariants and ultimately guide
% its synthesis.

Data-driven invariant synthesis techniques have gained considerable
traction in recent years.  Daikon~\cite{ernst2007daikon} is an early
and influential dynamic invariant generation tool.  It maintains a
pool of candidate invariants, which is repeatedly pruned upon
observing program executions. This approach has a few main
limitations: (1) it is sensitive to the initial set of candidate
invariants, (2) it is unable to identify complex invariants such as
those with disjunctions.

Counterexample guided invariant generation (CEGIR) techniques learn
safety invariants by using a combination of inductive synthesis and
verification.  For instance, the work on implication counterexample learning (ICE~\cite{garg2014ice} and ICE-DT~\cite{icedt}) is inspired
by computational learning theory; the authors use a learner and a
teacher, where the learner iteratively refines a candidate invariant
using counterexamples provided by the teacher until a valid invariant
is discovered. A central step is to include implications, which are counterexamples are not inductive by any reachable states, in
the learning algorithm that guarantee that the learned invariant is
inductive. Checking if a candidate invariant is inductive requires the
use of a model checker or an SMT solver. A limitation of ICE learning
is that the search space for invariants grows exponentially with the
number of variables and states, and that it requires model checking to
establish inductiveness of the invariant.

NumInv\cite{numinv} is a technique to automatically uncover complex
numerical invariants, sacrificing soundness for the ability to
discover numerical invariants effectively. NumInv also uses a model
checker to provide counterexamples and is primarily geared towards
deterministic sequential programs.

The work in
\cite{revisedFre}, a refined version of FreqHorn \cite{freqhorn}, conducts a
probabilistic search through candidate formulas and an efficient
counterexample-guided approach by encoding the problem of inductive synthesis as an SMT query. 

Some types of CEGIR work is domain-specific: In \cite{convexpoly} the
approach learns sound inductive invariants in the form of convex
polynomial inequalities. In \cite{nn}, the authors combine neural
networks with formal reasoning to synthesize loop invariants.
Code2Inv\cite{code2inv} employs a
graph neural network to represent the program structure and uses
reinforcement learning to explore candidate invariants.  ACHAR\cite{almostcorrect} employs the learner of the engine Code2Inv and reduces verification
of a program to test correctness of invariants using
testing-based reachability oracle, which is not  However, it also has the limitation of Code2Inv and with a theorem proving technique integrated. The work in
\cite{nonprovable} leverages CEGIR and non-provability information
provided by the verification engine.  


DistAI\cite{distai} is a recent approach designed to learn inductive
invariants of distributed protocols\cite{padon2016ivy} expressed in
the Ivy language using a data-driven approach. This approach requires
a safety property and the Ivy model checker. It uses a invariant
refinement process that is guided by detecting candidate invariants
that fail the Ivy model checker.  Candidate invariant refinement
relies on the predefined safety property and a model checker. If the
safety property does not hold for the protocol, DistAI may continue
the refinement loop forever. Similarly, DuoAI\cite{yao2022duoai} as the extension of DistAI to existential quantifiers also
relies on provided safety properties.  However, our tool solely replies on traces without safety properties provided. 

\noindent\textbf{Discussion and Future Work}
InvGen is an automated and practical framework for observing
non-deterministic system behaviors and generating accurate system
properties. The approach is data-driven, leveraging counter-examples
and speculative negative states to guide the refinement process. The
learning model is template-free and decision-tree-based. One key
advantage of our framework is its independence from any known system
specifications or properties.

Future work includes multiple promising directions. First, exploring
alternative speculative sampling techniques enhances the convergence
of the learning process. Second, the decision tree learning method
could be further investigated, including the separator selection and
the exploit-exploration trade-off.

